Probing the atmospheric precipitable water vapor with SOFIA, Part I, Measurements of the water vapor overburden with FIFI-LS

We report on the measurements of telluric water vapor made with the instrument FIFI-LS on SOFIA. Since November 2018, FIFI-LS has measured the water vapor overburden with the same measurement setup on each science flight with about 10 data points throughout the flight. This created a large sample of 469 measurements at different locations, flight altitudes and seasons. The paper describes the measurement principle in detail and provides some trend analysis on the 3 parameters. This presents the first systematic analysis with SOFIA based on in situ observations.

==> README <==
# harvard family of bibliographic styles
# Copyright 1994 - Peter Williams pwil3058@bigpond.net.au
#
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
# 
# The Current Maintainers of this work are Peter Williams and Thorsten Schnier.
#
# This work consists of all files listed in manifest.txt.
#
# Licence notice added on behalf of Peter Williams and Thorsten Schnier
# by Clea F. Rees 2009/01/30.

This is version 2.0.5 of the harvard family of bibliographic styles.
It is a bug fix of 2.0 which was a major rewrite to bring the sty file into
line with the new latex described in ``The LaTeX Companion''.  Due to the
efforts of Thorsten Schnier (thorsten@archsci.arch.su.edu.au) it incorporates
support for the LaTeX to html translator by Nikos Drakos
(nikos@cbl.leeds.ac.uk).

It includes a fixes by Berwin A. Turlach (berwin@alphasun.anu.edu.au) for
problems with \AtBeginDocument introduced in the latest version of LaTeX2e
and problems with the \nocite command.

A new style apsr.bst (American Political Science Review) is enclosed
courtesy of Nathaneil L. Beck (nbeck@weber.ucsd.edu)

NB.  The file harvard.sty makes considerable use of features in the new latex
that were not present in latex version 2.09 and is, therefore, not compatible
with that version.  However, the *.bbl files produced by the various bst files
should be still useable with latex version 2.09.

The following files are enclosed.

  README	- This file
  INSTALL	- Installation instructions
  Makefile	- Makefile for installation
  harvard.ps	- Postscript version of the documentation
  harvard.tex	- LaTeX source for the documentation
  harvard.bib	- BibTeX database file for the documentation
  doc_Makefile	- Makefile for documentation
  harvard.sty	- LaTeX style file for harvard bibliographic style
  harvard.perl	- LaTeX2html style file for harvard bibliographic style
  agsm.bst	- harvard BibTeX style file to satisfy the requirements
		  of the Australian Government Style Manual
  dcu.bst	- harvard BibTeX style file to satisfy the requirements
		  of the Design Computing Unit, Sydney University
  <other>.bst	- various style files contributed by users

Online documentation is available via the WWW at:

HREF="http://www.arch.su.edu.au/~peterw/latex/harvard/"

